A Geometry-Sensitive Quorum Sensing Algorithm for the Best-of-N Site Selection Problem

The house hunting behavior of the Temnothorax albipennis ant allows the colony to explore several nest choices and agree on the best one. Their behavior serves as the basis for many bio-inspired swarm models to solve the same problem. However, many of the existing site selection models in both insect colony and swarm literature test the model's accuracy and decision time only on setups where all potential site choices are equidistant from the swarm's starting location. These models do not account for the geographic challenges that result from site choices with different geometry. For example, although actual ant colonies are capable of consistently choosing a higher quality, further site instead of a lower quality, closer site, existing models are much less accurate in this scenario. Existing models are also more prone to committing to a low quality site if it is on the path between the agents' starting site and a higher quality site. We present a new model for the site selection problem and verify via simulation that is able to better handle these geographic challenges. Our results provide insight into the types of challenges site selection models face when distance is taken into account. Our work will allow swarms to be robust to more realistic situations where sites could be distributed in the environment in many different ways.

==> doc/model.tex <==
\section{Model}\label{sec:model}

We first describe a general discrete geographical model for modeling swarm agents. Then we discuss the individual restrictions, parameters, and agent algorithms needed for the house hunting problem specifically. 



\subsection{General Model}
We assume a finite set $R$ of agents, all of which have a state set $SR$ of potential states. Agents move on a discrete rectangular grid of size $n \times m$, formally modelled as directed graph $G = (V,E)$ with $|V| = mn$. Edges are  bidirectional, and we also include a self-loop at each vertex. Vertices are indexed as $(x, y)$, where $0 \leq x, y \leq n-1$. Each vertex also has a state set $SV$ of potential states.

We chose to use a discrete model so that sites could be easily defined in space and the model simulator could be run in a distributed fashion on each vertex to reduce computation time. 

\subsubsection{Model Configurations}
We define four kinds of configurations, global vs. local, and ordinary vs. transitory.  The transitory configurations are used as intermediate steps in defining system executions.  

\paragraph{(Global) configurations:}

A \emph{(global) configuration} $C$ is a triple of mappings, $(svmap, srmap, locmap)$, where:
\begin{itemize}
    \item 
    $svmap: V \rightarrow SV$ is the vertex state mapping, which assigns a vertex-state to each vertex,
    \item
    $srmap: R \rightarrow SR$ is the agent state mapping, which assigns an agent-state to each agent, and
    \item 
    $locmap: R \rightarrow V$ is the location mapping, which assigns a location to each agent.
\end{itemize}

\paragraph{Local configurations:}
A \emph{local configuration} $C'$ is intended to capture the contents of one vertex/square).  It is a triple $(sv, myagents, srmap)$, where:
\begin{itemize}
    \item 
    $sv \in SQ$ is the vertex-state of the given vertex,
    \item
    $myagents \subseteq R$ is the set of agents at the vertex, and
    \item 
    $srmap: myagents \rightarrow SR$ assigns an agent-state to each agent at the vertex.
\end{itemize}

Define an operator $project(C,v)$, which takes a global configuration $C$ and projects it to give a local configuration of vertex $v$.
Namely, if $C = (svmap, srmap, locmap)$, and $v$ is any vertex, then $project(C,v)$ is the local configuration
$(svmap(v), R', srmap \lceil R')$, where $R' = \{r \in R : locmap(r) = v\}$.
That is, we pick out the state of the given vertex $v$, and the states for all the agents located at $v$.

We also define an inverse operation called $merge$, which combines local configurations to yield a global configuration.
We assume a collection of "compatible" local configurations 
$\{C'(v) : v \in V \}$, where "compatible" here means that the unique vertices below exist.
The resulting global configuration $C$ is defined by:
\begin{itemize}
    \item 
    For every $v \in V$, $svmap(v) = C'(v).sv$, that is, take the state of $v$ from the local configuration belonging to vertex $v$.
    \item
    For every $r \in R$, $locmap(r)$ is the unique vertex $v$ such that $r \in C'(v).myagents$, and $srmap(r) = C'(locmap(r)).srmap(r)$.
\end{itemize}

\subsubsection{Transitory Configurations}
We also have a notion of transitory configuration, which is used as an intermediate stage between two ordinary configurations, in constructing executions.  It represents agents in motion from one vertex to another. 

A \emph{transitory configuration} $T$ is a triple of mappings $(svmap, srmap, edgemap)$, where
\begin{itemize}
\item
$svmap$ and $srmap$ have the same types as for ordinary configurations, and
\item
$edgemap: R \rightarrow E$ assigns a directed edge to each agent.
\end{itemize}

This represents newly-computed states for all vertex and agents, plus the edges on which the agents are traveling to get to their next locations.

\paragraph{Local transitory configurations:}
A \emph{local transitory configuration} $T'$ is a quadruple $(sv, myagents, srmap, dirmap)$, where
\begin{itemize}
\item 
$sv$, $myagents$, and $srmap$ are as in the definition of a local configuration, and
\item
$dirmap: myagents \rightarrow \{R,L,U,D,S\}$ is the direction mapping, which assigns a travel direction to each agent.  Direction $S$ means to stay at the vertex.
\end{itemize}
This represents newly-computed states for a single vertex and its agents, plus directions of travel for the local agents.

As before, define an operator $project(T,v)$, which takes a global transitory configuration $T$ and projects it to give a local transitory configuration $T(v)$ for vertex $v$.
Namely, if $T = (svmap, srmap, edgemap)$, and $v$ is any vertex, then $project(T,v)$ is the local transitory configuration
$(svmap(v), myagents, srmap \lceil myagents, dirmap)$,
where:
\begin{itemize}
\item
$myagents = \{r \in R : edgemap(r) \mbox{ is an edge with } source = v \}$, and
\item
For each $r \in myagents, dirmap(r)$ is the direction of the edge $edgemap(r)$, that is, $R$ if the edge goes from $v$ to its right neighbor, etc.
\end{itemize}

We also define an inverse, $merge$ operation, which combines local transitory configurations to give a global transitory configuration.
We assume a collection of "compatible" local configurations $\{T'(v) : v \in V\}$, where "compatible" means that the unique vertices below exist.  
The resulting global transitory configuration $T$ is defined by:
\begin{itemize}
    \item 
    For every $v \in V$, $svmap(v) = T'(v).sv$,
\item
For every $r \in R$, let $v$ be the unique vertex such that $r \in T'(v).myagents$; then define:
\begin{itemize}
    \item $srmap(r) = T'(v).srmap(r)$.
    \item $edgemap(r)$ is the directed edge from $v$ to $w$, where $w$ is the vertex that is the target of the edge from $v$ in the direction given by $T'(v).dirmap(r)$.
\end{itemize}
\end{itemize}

Given a transitory configuration $T = (svmap, srmap, edgemap)$, we can map it to an ordinary configuration using $C = move(T)$ , which is the same as $T$ except that, instead of edgemap, we have locmap, where for each $r \in R$, $locmap(r) = target(edgemap(r))$.

\subsubsection{Local transitions}
The transition of a vertex $v$ may be influenced by the local configurations of nearby vertices in addition to itself. We define an \textbf{influence radius} $I$, which is the same for all vertices, to mean that vertex indexed at $(x,y)$ is influenced by all vertices $\{(a,b) | a \in [x-I, x+I], b\in [y-I, y+I]\}$, where $a$ and $b$ are integers mod $n$. 
We can use this influence radius to create a local mapping $M_v$ from local coordinates to the neighboring local configurations. Thus, for a vertex $v$ at location $(x,y)$, we produce $M_v$ such that $M_v(a,b) \rightarrow C'(w)$ where $w$ is the vertex located at $(x+a, y+b)$ and $ -I < a,b < I$. This influence radius is representative of a sensing and communication radius for agents.

We have a local transition function $\delta$, which maps all the information associated with one vertex and its influence radius at one time to new information that can be associated with the vertex at the following time.  It also produces directions of motion for all the agents at the vertex.

Formally, for a vertex $v$, $\delta$ maps the mapping $M_v$ to a probability distribution on local transitory configurations of the form $(sv_1, myagents, srmap_1, dirmap_1)$, where:
\begin{itemize}
\item
$sv_1 \in SV$ is the new state of the vertex,
\item
$srmap_1: myagents \rightarrow SR$ is the new agent state mapping, for agents currently at the vertex, and
\item
$dirmap_1: myagents \rightarrow \{R,L,U,D,S\}$ gives directions of motion for all the agents currently at the vertex.
\end{itemize}

\subsubsection{Local transition function $\delta$}
The local transition function $\delta$ is further broken down into two phases as follows.
\paragraph{Phase One:} Each agent in vertex $v$ uses the same probabilistic transition function $\alpha$, which maps the agent's state $sr \in SR$, location $(x,y)$, the vertex state of the location $sv \in SV$, and the mapping $M_v$ to a distribution over new suggested vertex state $sv'$, agent state $sr'$, and direction of motion $d \in \{R, L, U, D, S\}$.
\paragraph{Phase Two:} A rule $L$ is used to reconcile the different vertex states suggested by each agent at the vertex and select one final vertex state. The rule also determines for each agent whether they may transition to state $sr'$ and direction of motion $d$ or stay at the same location with original state $sr$.

\subsubsection{Probabilistic execution}

The system executes probabilistically, moving through an infinite sequence of configurations $C_0, C_1, C_2,\ldots,$ each derived probabilistically from the previous one.

We first describe how the system moves from any configuration $C_t$ to the next configuration $C_{t+1}$.
This is a two-phase process where the first phase is probabilistic and the second is deterministic.
The first phase yields a transitory configuration, and the second phase converts that to an ordinary configuration.

\paragraph{Phase 1:}
For each vertex $v$ independently, use $project(C_t,w)\ \forall w \in IR(v)$ to obtain the local mapping $M_v$.
Then apply $\delta$ to $M_v$, and sample the resulting distribution to select a local transitory configuration for $v$.  
Apply $merge$ to combine these independent results for all $v$ as described above, to obtain a global transitory configuration.

\paragraph{Phase 2:}
For the transitory configuration $T$ resulting from Phase 1, compute $move(T)$ to get the new configuration.

\subsection{House Hunting Model}
The goal of the house hunting problem is for agents to explore the grid and select the best of $S$ sites to migrate to collectively. We model sites as follows. 

A set $S$ of square-shaped sites are located within this grid, where site $s_i$ has lower left vertex $(x_i^1, y_i^1)$ and upper right vertex $(x_i^2, y_i^2)$. Each site $s_i$ also has a quality $s_i.q \in [0,1]$. To represent these sites, we let the vertex state set be $SV = S \cup \{\emptyset \}$ for each vertex, indicating that each vertex can either be part of one or zero sites. Furthermore, we denote the site $s_0$ to be the \textit{home nest}. In the initial configuration, all agents start out randomly at one of the vertices of the home nest. 

\subsection{Agent states and transition function}
The agent state set $SR$ is best described in conjunction to the agent transition function $\alpha$. Agents can take on one of $6$ different core states, each of them a combination of one of three preference states (Uncommitted, Favoring, Quorum), and two activity states (Nest, Active). 

Uncommitted Nest ($U^N$) agents stay in the home nest in order to prevent too many agents from flooding the environment. They have a chance of transitioning to Uncommitted Active ($U^A$) agents, which try to explore the arena and discover new sites. Uncommitted Active agents move according to the Levy flight random walk, which has been shown to be used by foraging ants in nature \cite{sims2012levy}. Uncommitted Nest agents transition to Active with probability $P_A$, and Uncommitted Active agents transition to nest agents with probability $P_N$. This ensures that $\frac{P_A}{P_A+P_N}$ percent of uncommitted agents are active, whereas $\frac{P_N}{P_A+P_N}$ agents remain in the nest. Prior work lets $P_N = 9P_A = L$, where $L$ is the inverse of the average site round trip time, chosen to promote sufficient mixing. This leads to $10\%$ of the agent population being active.

Uncommitted Active agents have a chance of discovering a new nest. If they do so, they explore the nest and accept it with probability $s_i.q$, where $s_i.q$ is the quality of nest $i$. They then have an $x = \frac{P_A}{P_A+P_N}$ chance of transitioning to Favoring Active, and a $1-x$ chance of transitioning to Favoring Nest. 

Favoring Active $(F^A)$ agents have discovered a nest that they favor and remain in the nest to build quorum for it. Favoring Nest $(F^N)$ agents have discovered a nest that they favor and are returning to the home nest to recruit others. Favoring Nest agents transition to Active with the same probability $P_A$ and Favoring Active agents transition back to Nest agents with probability $P_N$, creating the same effect where $90\%$ of the agent population is actively recruiting while the rest remain in the favored nest to try and build up quorum.

Favoring Active agents have a probability $\alpha$ of abandoning their nest, which is set to 1 if the time spent without encountering any other agents surpasses $t_\alpha$. Favoring Nest agents have a chance of being inhibited by other Favoring Nest agents. The chance an agent favoring nest $i$ is converted to favoring nest $j$ is $D r_j C_{ij}$, where the factor of $D$ is a message delay to simulate the probability of agents sending eachother so that excessive messaging does not occur. $r_j$ is the number of agents favoring site $j$ within sensing radius. After an agent hears of a new potential site $j$, it visits the site itself to evaluate the quality and changes its preference if it deems the new site to be better than it's preferred site. Therefore the condition $C_{ij}$ is $1$ when the agent evaluates site $j$ to be higher than site $i$ and $0$ otherwise. 

Active Uncommitted agents and Active Favoring agents can detect a quorum in a site when $q$ other agents in the site are within sensing range. The quorum function scales with site value as $q = \lfloor(q_{MIN}-q_{MAX})*s_i.q + q_{MAX} \rfloor$, where $q_{MAX}$ and $q_{MIN}$ are the maximum and minimum possible quorum threshold respectively. The condition $C_Q$ is $1$ when quorum is satisfied and $0$ otherwise. Agents from any Favoring or Uncommitted state also have a chance of transitioning into quorum state, if they encounter an agent already in quorum. The condition $C_{Q_i}$ is $1$ when another quorum agent for site $i$ is encountered and $0$ otherwise. Furthermore, agents have an $x = \frac{P_A}{P_A+P_N}$ chance of transitioning to Quorum Active and a $1-x$ chance of quorum nest after having detected or been notified of a quorum. 

Quorum Nest agents head to the home nest to inform others of the move, while Quorum Active agents randomly wander the grid to find stragglers. Agents in quorum states continue to wander until they have sensed quorum for $t_Q$ time steps, whereupon they return to the new selected site. 

The resulting agent state set $SR$ is therefore a product of the $6$ core states needed in the state machine model as well as a number of intermediate variables such as an agent's destination, the names of the sites it favors or has sensed quorum for, parameters for an agent's random walk when exploring the grid, and more. 

The transition function $\alpha$, which for each agent returns a proposed new vertex state $sv'$, agent state $sr'$ and direction of motion works as follows. Since in the house hunting problem (unlike other problems like task allocation), an agent never modifies the environment, $sv'=sv$ (the proposed new vertex state is always the same as the old vertex state). The agent state $sr'$ and direction $d$ are calculated according to the core transitions and the smaller state variables needed to keep track of those transitions. For example, when an agent is headed towards a site, the direction $d$ is calculated to try to match a straight-line traversal to the site from the agent's starting location as close as possible. 

